On the Feasibility of Out-of-Band Spatial Channel Information for Millimeter-Wave Beam Search

The rollout of millimeter-wave (mmWave) cellular network enables us to realize the full potential of 5G/6G with vastly improved throughput and ultra-low latency. MmWave communication relies on highly directional transmission, which significantly increase the training overhead for fine beam alignment. The concept of using out-of-band spatial information to aid mmWave beam search is developed when multi-band systems operating in parallel. The feasibility of leveraging low-band channel information for coarse estimation of high-band beam directions strongly depends on the spatial congruence between two frequency bands. In this paper, we try to provide insights into the answers of two important questions. First, how similar is the power angular spectra (PAS) of radio channels between two well-separated frequency bands? Then, what is the impact of practical system configurations on spatial channel similarity? Specifically, the beam direction-based metric is proposed to measure the power loss and number of false directions if out-of-band spatial information is used instead of in-band information. This metric is more practical and useful than comparing normalized PAS directly. Point cloud ray-tracing and measurement results across multiple frequency bands and environments show that the degree of spatial similarity of beamformed channels is related to antenna beamwidth, frequency gap, and radio link conditions.

==> acro_list.tex <==
\begin{acronym}[MU-MIMO] % Give the longest label here so that the list is nicely aligned
\acro{2D}{two-dimensional}
\acro{3D}{three-dimensional}
\acro{3GPP}{third generation partnership project}
\acro{3G}{third generation}
\acro{4G}{fourth generation}
\acro{5G}{fifth generation}
\acro{6G}{sixth generation}
\acro{AoA}{azimuth angle of arrival}
\acro{AoD}{azimuth angle of departure}
\acro{AC}{anechoic chamber}
\acro{A/D}{analog to digital}
\acro{BB}{base band}
\acro{BS}{base station}
\acro{CC}{coaxial cable}
\acro{CDF}{cumulative distribution function}
\acro{CDL}{clustered delay line}
\acro{CE}{fading channel emulator}
\acro{CFR}{channel frequency response}
\acro{CIR}{channel impulse response}
\acro{CWC}{Centre for Wireless Communications}
\acro{D/A}{digital to analog}
\acro{D2D}{device to device}
\acro{DFT}{discrete Fourier transform}
\acro{DPS}{Doppler power spectrum}
\acrodefplural{DPS}{Doppler power spectra}
\acro{DUT}{device under test}
\acro{EM}{electro-magnetic}
\acro{EoD}{elevation angle of departure}
\acro{FDD}{frequency division duplex}
\acro{FIR}{finite impulse response}
\acro{FR1}{Frequency Range 1}
\acro{FR2}{Frequency Range 2}
\acro{GSCM}{geometry-based stochastic channel model}
\acro{HPBW}{half power beam width}
\acro{HW}{hardware}
\acro{iid}{independent identically distributed}
\acro{I/O}{input/output}
\acro{IF}{intermediate frequency}
\acro{ITU-R}{International telecommunication union - Radiocommunication section}
\acro{LOS}{line of sight}
\acro{LTE}{Long Term Evolution}
\acro{MIMO}{Multiple-Input-Multiple-Output}
\acro{mm-wave}{millimetre wave}
\acro{MPAC}{multi-probe anechoic chamber}
\acro{MRC}{maximal ratio combining}
\acro{MU-MIMO}{multi-user MIMO}
\acro{NLOS}{non-line of sight}
\acro{OLOS}{obstructed line of sight}
\acro{OTA}{over the air}
\acro{PADP}{power angular delay profile}
\acro{PAS}{power angular spectrum}
\acrodefplural{PAS}{power angular spectra}
\acro{PDF}{probability distribution function}
\acro{PDP}{power delay profile}
\acro{PM}{phase matrix}
\acro{PSP}{PAS similarity percentage}
\acro{RC}{reverberation chamber}
\acro{RF}{radio frequency}
\acro{RIS}{reconfigurable intelligent surface}
\acro{RMS}{root mean squared}
\acro{RoF}{RF over fibre}
\acro{RRM}{radio resource management}
\acro{RTS}{radiated two-stage}
\acro{Rx}{receiver}
\acro{SINR}{signal to interference plus noise power ratio}
\acro{SIR}{signal to interference power ratio}
\acro{SISO}{Single-Input-Single-Output}
\acro{SNR}{signal to noise power ratio}
\acro{SW}{software}
\acro{TDD}{time division duplex}
\acro{TDL}{tapped delay line}
\acro{Tx}{transmitter}
\acro{UE}{user equipment}
\acro{ULA}{uniform linear array}
\acro{WC}{wireless cable}
\acro{WSS}{wide sense stationary}
\acro{WRC}{World Radiocommunication Conference}
\acro{ZF}{zero forcing}
\acro{}{}
\end{acronym} 
